ComplexCodeEval: A Benchmark for Evaluating Large Code Models on More Complex Code

In recent years, the application of large language models (LLMs) to code-related tasks has gained significant attention. However, existing evaluation benchmarks often focus on limited scenarios, such as code generation or completion, which do not reflect the diverse challenges developers face in real-world contexts. To address this, we introduce ComplexCodeEval, a benchmark designed to assess LCMs in various development tasks, including code generation, completion, API recommendation, and test case generation. It includes 3,897 Java samples and 7,184 Python samples from high-star GitHub repositories, each annotated with function signatures, docstrings, and API references to simulate real development environments. Our experiments across ten LCMs reveal that context improves performance and that data leakage can lead to overestimation, highlighting the need for more accurate evaluations.

==> 7_related_work.tex <==
\section{Related Work}

% In recent years, the field of code generation has seen significant advancements, driven by the development of various benchmarks to evaluate the performance of large language models. Early benchmarks like HumanEval \cite{chen2021evaluating} and MBPP \cite{austin2021program} primarily focused on generating Python code from natural language descriptions. APPS \cite{hendrycks2021measuring} extended this by evaluating models on more complex, competition-style problems, while ClassEval \cite{du2023classeval} assessed class-level code generation.

% To address more complex scenarios, benchmarks such as DS-1000 \cite{lai2023ds} and Concode \cite{iyer2018mapping} introduced non-standalone programs and data science API generation tasks. CoderEval \cite{yu2024codereval} further expanded the evaluation scope by incorporating non-standalone programs with contextual dependencies, providing a more comprehensive assessment of code generation capabilities.

% Recent benchmarks, including EvoCodeBench \cite{li2024evocodebench} and LiveCodeBench \cite{jain2024livecodebench}, have aligned more closely with real-world code repositories and offer detailed annotations. EvoCodeBench emphasizes mitigating data leakage and is dynamically updated. LiveCodeBench captures various facets of code reasoning and generation through continuous updates and a diverse set of tasks, such as code repair, code execution, and test output prediction.

% \textbf{Large Code Models}
% Codellama\cite{roziere2023code} is a family of code language models fine-tuned based on Llama 2. It supports functionalities such as code completion and code generation, and extends the context window to a size of 16k. DeepSeek-Coder\cite{guo2024deepseek}, developed by DeepSeek, is a series of open-source code models that support multiple programming languages and project-level code generation and completion. Its training data comprises 2T tokens, with 87\% consisting of code and 13\% consisting of natural language. StarCoder 2\cite{lozhkov2024starcoder} is part of the BigCode project and includes code generation models of three different sizes: 3B, 7B, and 15B. These models are trained on over 600 programming languages and some natural language texts, enabling them to generate, analyze, and document code. StarCoder 2 performs exceptionally well among open-source code LLMs, surpassing its predecessor, StarCoder\cite{li2023starcoder}.

% \textbf{Benchmarks}
HumanEval\cite{chen2021evaluating} is a commonly used benchmark for evaluating code generation, containing 164 handwritten natural language descriptions and test cases. HumanEval-X\cite{zheng2023codegeex} builds on HumanEval by adding multiple programming languages (C++, Java, JavaScript, Go). CoderEval\cite{yu2024codereval} collects 230 samples each of Java and Python from GitHub repositories and manually constructs projects to test the code generated by LCMs. CrossCodeEval\cite{ding2023crosscodeeval} is a benchmark for evaluating the cross-file, line-level code completion capabilities of LCMs. This dataset is automatically collected from GitHub and includes four programming languages, using Exact Match (EM) and Edit Similarity (ES) as evaluation metrics. APIBench\cite{peng2021revisiting} includes datasets for evaluating two types of API recommendation tasks: query-based and code-based, named APIBench-Q and APIBench-C, respectively. For the test case generation task, method2test\cite{tufano2020unit} is a dataset containing Java methods and corresponding test cases, with its test set comprising 78,388 instances from 1,017 repositories.


==> 8_threats_to_validity.tex <==
\section{Threats To Validity}

\textbf{Threats in Benchmark Construction.} One potential threat is the way how we record the timestamps of the selected repositories. Due to the possibility of not obtaining the corresponding time information from git commit records, we adopted a fallback mechanism: when the file creation time is unavailable, we use the project creation time as the file creation time; when the update time is unavailable, we use the creation time as the update time. This fallback mechanism may unintentionally introduce some level of bias when examining the effect of data leakage. Another threat is that there may be room for improvement in the automatically generated docstrings. More advanced generation strategies (e.g., controlled text generation \cite{dekoninck2023controlled}) could be used to improve the quality of the docstrings. \textbf{Threats in Empirical Study.} Due to computing resource constraints, as of the writing of this paper, we have not yet conducted experiments on more open-source models (e.g., CodeGeex \cite{zheng2023codegeex}, WizardCoder \cite{luo2023wizardcoder}) and closed-source models (e.g., ChatGPT \cite{OpenAI2023}). Additionally, to incorporate various contextual information, we used specifically formatted prompts, which may affect the experimental results.
